Graph Sanitation with Application to Node Classification

The past decades have witnessed the prosperity of graph mining, with a multitude of sophisticated models and algorithms designed for various mining tasks, such as ranking, classification, clustering and anomaly detection. Generally speaking, the vast majority of the existing works aim to answer the following question, that is, given a graph, what is the best way to mine it? In this paper, we introduce the graph sanitation problem, to answer an orthogonal question. That is, given a mining task and an initial graph, what is the best way to improve the initially provided graph? By learning a better graph as part of the input of the mining model, it is expected to benefit graph mining in a variety of settings, ranging from denoising, imputation to defense. We formulate the graph sanitation problem as a bilevel optimization problem, and further instantiate it by semi-supervised node classification, together with an effective solver named GaSoliNe. Extensive experimental results demonstrate that the proposed method is (1) broadly applicable with respect to different graph neural network models and flexible graph modification strategies, (2) effective in improving the node classification accuracy on both the original and contaminated graphs in various perturbation scenarios. In particular, it brings up to 25% performance improvement over the existing robust graph neural network methods.

==> Files/04Framework.tex <==
% \section{Q-Learning Based Solution}
% \label{sec:framework}

% Based on the problem setting and discussion in Sec. \ref{sec:problemDefinition}, the active defense problem defined as Eq.~\eqref{eq:active defense objective function} can generalize to a wide range of problems by the combination of different defenders and attackers. In this paper, we study the problem on topology attack and defense, and leave the other topics as future work. For most graph data, the topology of the graph is represented as a binary adjacency matrix, which means only discrete topology modification is practicable for the defender. For modelling the discrete actions of defender, we adopt the deep Q network with replay memory~\cite{mnih2015human} as the backbone of our framework as we shown in Figure~\ref{fig:framework}.

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[scale=0.2]{Figures/Framework.png}
% 	\caption{The framework of our active defense strategy based on reinforcement learning.}
% 	\label{fig:framework}
% \end{figure}

% In general, the procedure of modifying the graph from the defender is modeled as a finite horizon markov decision process whose length is limited by the defending budget $\Delta_d$. In every step the defender makes an action (modification) on the half-done defended graph and the environment containing a simulated attacker strategy would perform an adversarial attack on the defended graph (by increasing the loss of a target model) to get an attacked graph. Finally, the environment evaluates the effectiveness of modification based on the outputs of target model fed with benign graph and defended-then-attacked graph, respectively. It is worth mentioning that even though the goal of our framework is to retain the performance of classifier on all the defended-then-attacked unlabeled nodes, it is infeasible due to the giant action space and unstable convergence (e.g. the accuracy over all the unlabeled node may change slightly which can mislead the training). Hence, the goal for the defender is to learn how to retain the performance of classifier on the defended-then-attacked target nodes ($\mathcal{V}_{t}\in\mathcal{V}$), and in the following section we will show that by a tricky selection of the target nodes, the robustness over all the unlabeled node can be improved. Next, we will introduce the components of our proposed framework.
% % In order to follow the 'small modification' constraint~\cite{dai2018adversarial}, not only the length of modification process is limited by the defending budget $\Delta_d$, the 


% % From the perspective as a defender, we aim to use a simulated attacker to execute the attack on the defended graph (during testing period, i.e. evasion attack) in order to offer feedback towards the defense operation.
% % The whole framework could be summarized as follows:

% % \begin{itemize}
% %     \item Initialization 1: Train a model $\theta_{G}^{*}$ (i.e. semi-supervised node classifier) on the labelled nodes in a benign graph $G$ based on $\theta^{*}_{G}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(G),\mathbf{z})$.
% %     \item Initialization 2: Obtain the original output on unlabelled nodes in the benign graph $G$ as $f_{\theta_{G}^{*}}(G)$
% %     \item Step 1: Modify the benign graph $G$ by a defender model and output $G_d$.
% %     \item Step 2: Train another model $\theta_{G_d}^{*}$ (i.e. semi-supervised node classifier) on the labelled nodes in a modified graph $G_d$ based on $\theta^{*}_{G_d}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(G_d),\mathbf{Z})$
% %     \item Step 3: Use a simulated attacker model to execute topology attack and output $\tilde{G_d}$.
% %     \item Step 4: Obtain the output on unlabelled nodes in the defended and attacked graph $\tilde{G_d}$ as $f_{\theta_{G_d}^{*}}(\tilde{G_d})$
% %     \item Step 5: Update the defender model based on $f_{\theta_{G_d}^{*}}(\tilde{G_d})$ and $f_{\theta_{G}^{*}}(G)$
% % \end{itemize}

% % \begin{algorithm}[t]
% % \caption{Framework of Active Topology Defense}
% %     \begin{algorithmic}[1]
% %         \INPUT (1) a benign graph $G$ with part of labels $\mathbf{z}$, (2) a classifier $f$ with parameter $\theta$ (3) a simulated attacker model.
% %         \OUTPUT (1) a defended graph $G_d$.

% %         \State Initialization: (1) Train a model $\theta_{G}^{*}$ (i.e. semi-supervised node classifier) on the labelled nodes in a benign graph $G$ based on $\theta^{*}_{G}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(G),\mathbf{z})$; (2) Obtain the original output on unlabelled nodes in the benign graph $G$ as $f_{\theta_{G}^{*}}(G)$.
    
% %         \While {not converged}
% %             \State Modify the benign graph $G$ by a defender model and output $G_d$.
% %             \State Train another model $\theta_{G_d}^{*}$ (i.e. semi-supervised node classifier) on the labelled nodes in a modified graph $G_d$ based on $\theta^{*}_{G_d}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(G_d),\mathbf{Z})$.
% %             \State Use a simulated attacker model to execute topology attack and output $\tilde{G_d}$.
% %             \State Obtain the output on unlabelled nodes in the defended and attacked graph $\tilde{G_d}$ as $f_{\theta_{G_d}^{*}}(\tilde{G_d})$
% %             \State Update the defender model based on $f_{\theta_{G_d}^{*}}(\tilde{G_d})$ and $f_{\theta_{G}^{*}}(G)$.
% % 		\EndWhile
% % 		\State \Return $G_d$
% %     \end{algorithmic}
% % \label{alg: framework}
% % \end{algorithm}

% % In order to formulate every steps during the training, we armed them into a deep Q network, i.e. a finite horizon markov decision process ($S,A,P,R,\gamma$).

% \subsection{State}
% \label{sec:state}
% %  We first learn the node embedding based on struct2vec~\cite{dai2016discriminative}
% In order to fully represent the status of half-done defended graph, we use the embedding of the graph $G_d^t$ at time $t$ and the embedding of target node set $\mathcal{V}_t$ to compose the state vector $\mathbf{s}^t$. At first, we use a GCN-styled encoder to perform node embedding whose output is as follows:
% \begin{equation}
%     \mathbf{E} = \textrm{ReLU}\Big(\hat{\mathbf{A}_d^t}\mathbf{X}\mathbf{W}^{(0)}\Big)\mathbf{W}^{(1)},
% \end{equation}
% \noindent where the notation definitions are same as we introduced Eq.~\eqref{eq:GCN output} except $\hat{\mathbf{A}_d^t}$ which is the normalized laplacian matrix of the half-done defended graph $G_d^t$. The embedding vector $\mathbf{e}(v_i)$ of the $i$-th node $v_i$ can be obtained through indexing the output matrix $\mathbf{E}$ as $\mathbf{e}_i=\mathbf{E}[i,:]$.
% Then, we obtain the state representation as:
% \begin{equation}
%     \mathbf{s}^t = \mathbf{e}_t||\mathbf{e}_g,
% \label{eq:state function}
% \end{equation}
% % \begin{equation}
% %     \mathbf{s}^t = \sum_{v_i\in\mathcal{V}}\frac{\mathbf{e}(v_i)}{|\mathcal{V}|}
% % \end{equation}
% \noindent where the $||$ is the concatenation operator, $\mathbf{e}_t=\sum_{v_i\in\mathcal{V}_t}\frac{\mathbf{e}(v_i)}{|\mathcal{V}_t|} $ and $\mathbf{e}_g=\sum_{v_i\in\mathcal{V}}\frac{\mathbf{e}(v_i)}{|\mathcal{V}|}$ are target nodes embedding and graph embedding respectively as average pooling of node embeddings over corresponding node set.

% \subsection{Action}
% Goal of the defender (i.e. agent) is to defense (i.e. modify) the topology of benign graph in order to retain the performance of classifier over the defended-then-attacked target nodes $\mathcal{V}_t$. Specifically, action the defender makes is to flip the entries of adjacency matrix, i.e. deleting or adding an edge. At every time step, the defender select a pair of nodes $(v_a^{(0)},v_a^{(1)})$ and deleting the edge between them if there is already an edge. Otherwise, adding an edge between the node pair. Thus, the action can be represented by the node pair $(v_a^{(0)},v_a^{(1)})$ whose encoding is as follows:

% \begin{equation}
%     \mathbf{a}^t = \mathbf{e}(v_a^{(0)})||\mathbf{e}(v_a^{(1)}),
% \label{eq:action function}
% \end{equation}

% \noindent where the embedding vector is indexed by the embedding matrix introduced in Sec. ~\ref{sec:state}. As aforementioned, the modification from defender should also follows the “small modification” constraint~\cite{dai2018adversarial}. Hence, not only the number of time steps is limited by defensing budget, the action node pair $(v_a^{(0)},v_a^{(1)})$ at every time step should be selected from the union of $n$-hop neighbors of all the target nodes $\mathcal{V}_t$. 
% % that the classifier would perform similarily given We designate the defender as the agent in this reinforcement learning framework whose action is adding a new edge or deleting an existing edge. We encoding the action at time $t$ as $\mathbf{a}^t$ with following form:

% % There has an option that we could encode the deleting or the adding operation ($o$) in it:
% % \begin{equation}
% %     \mathbf{a}^t = [e(v_{source})||e(v_{target})||o].
% % \end{equation}

% \subsection{Policy Network}
% We use a deep Q network to evaluate the long-term reward for the actions taken by the defender at each time step. The famous Bellman equation describes the property of optimal action-value function $Q^*(\mathbf{s}^t,\mathbf{a}^t)$ as follows~\cite{mnih2015human}:

% \begin{equation}
%     Q^*(\mathbf{s}^t,\mathbf{a}^t)=r(\mathbf{s}^t,\mathbf{a}^t)+\gamma\max_{\mathbf{a}^{t+1}}Q^*(\mathbf{s}^{t+1},\mathbf{a}^{t+1}).
% \end{equation}
% \noindent where $r$ is the reward from action $\mathbf{a}^t$ under state $\mathbf{s}^t$, $gamma$ is the discount hyperparameter.

% In this paper we model action-value function via a two-layer neural networks as follows,
% \begin{equation}
%     Q(\mathbf{s}^t,\mathbf{a}^t)=\mathbf{W}^{(1)}_{Q}\ \textrm{ReLU}(\mathbf{W}^{(0)}_{Q}(\mathbf{s}^t||\mathbf{a}^t)).
% \end{equation}

% % Given the current $Q$, the agent selection the next action $\mathbf{a}^t$ based on the following formula:
% For a given action-value function, the defender select the action greedily by maximizing the expected Q value as follows:
% \begin{equation}
%     \mathbf{a}^t = \arg\max_{\mathbf{a}}Q(\mathbf{s^t},\mathbf{a}).
% \label{eq:greedy selection}
% \end{equation}
% % \noindent During training period, we import a commonly-used decay-with-iteration probability $\epsilon$ to decide if the defender takes greedy action or random action.

% \subsection{Reward}
% As we shown in the framework in Figure \ref{fig:framework}, the simulated attacker is a part of the environment to give feedback to defender about the effectiveness of action that the defender takes each time step. The direct inspiration for such a simulated attacker is the so-called black box attack and attack transferability~\cite{papernot2016transferability} which illustrate that an attacked test sample from a specific model can also fool other models trained on the same training set. The intuitive explanation of their observation is that the decision boundaries of different classifiers trained on the same training data have common defects, so when a test sample is attacked and moved into another side of a specific decision boundary (i.e. successful attack), presumably it was moved into another side of other decision boundaries (for other classifiers) as well. Thus, we have an assumption that the manners of different attacker models for a specific test data should share common ground. If the test data is moved far away from the decision boundary and be robust for a specific attacker, it would be robust and hard-to-attack for other attackers as well.

% Based on the above idea, our framework assigns reward to the action at each time step based on the following criteria:

% \begin{equation}
% r(\mathbf{s}^t,\mathbf{a}^t) = 
% \left\{
%     \begin{array}{ll}
%       1; & \textrm{if}\ B(\mathbf{s}^t,\mathbf{a}^t)>0 ,\\
%       -1 ; & \textrm{otherwise}.\\
%     \end{array}
% \right.
% \label{eq:reward function}
% \end{equation}

% \noindent where $B$ is the action defense gain defined as follows:

% \begin{equation*}
%     B(\mathbf{s}^t,\mathbf{a}^t) = \mathcal{D}(f_{\theta^{*}_{G}}(G),f_{\theta^{*}_{G_{d}^{t+1}}}(\tilde{G_d^{t+1}})) - \mathcal{D}(f_{\theta^{*}_{G}}(G),f_{\theta^{*}_{G_{d}^{t}}}(\tilde{G_d^{t}})).
% \end{equation*}

% \noindent The key idea of the action defense gain is to compare the output of target classifier fed with defended-then-attacked graph with its output fed with benign graph. If the action taken at time step $t$ reduces the distance between output fed with defended-then-attacked graph and output fed with benign graph, the action defense gain is positive, and the reward for action at time step $t$ is $1$. Otherwise, the reward is $-1$. Remarks that as we stated at the beginning of Sec. \ref{sec:framework}, we focus on the defense performance towards the target nodes $\mathcal{V}_t$ for stable training. Thus, outputs (i.e. $f_{\theta^{*}_{G}}(G)$, $f_{\theta^{*}_{G_{d}^{t+1}}}$, $f_{\theta^{*}_{G_{d}^{t}}}$) compared in formula $B(\mathbf{s}^t,\mathbf{a}^t)$ are all indexed by node set $\mathcal{V}_t$.

% Since the simulated attacker needs to attack the half-done defended graph every time step, in this paper, we select fast gradient sign method (FGSM)~\cite{goodfellow2014explaining} as the simulated attacker for its great efficiency and effectiveness. However, for FGSM~\cite{goodfellow2014explaining}, it is first introduced to perturb image input with continuous feature space, and though papers like~\cite{zugner2018adversarial} have some trials to use FGSM to attack graph data, their solutions are not effective and suitable for our scenario. As our framework does not require a valid attacked output (i.e. attacked graph with binary adjacency matrix) but only needs to test the robustness of defended graph, we directly conduct FGSM on the normalized laplacian matrix of defended graph and use the attacked laplacian matrix as input to our target classifier.
% % At first we define the defensive benefit $B$ in time step $t$ as the difference between attacked results in two time steps $t+1$ and $t$ when the defender takes action $\mathbf{a}^t$ as follows,
% % \begin{equation}
% %     B(\mathbf{s}^t,\mathbf{a}^t) = \mathcal{D}(f_{\theta^{*}_{G}}(G),f_{\theta^{*}_{G_{d}^{t+1}}}(\tilde{G_d^{t+1}})) - \mathcal{D}(f_{\theta^{*}_{G}}(G),f_{\theta^{*}_{G_{d}^{t}}}(\tilde{G_d^{t}}))
% % \end{equation}

% % We set the reward as the sign of defensive benefit in time step $t$ as follows,
% % \begin{equation}
% % r(\mathbf{s}^t,\mathbf{a}^t) = 
% % \left\{
% %     \begin{array}{ll}
% %       1; & \textrm{if}\ B(\mathbf{s}^t,\mathbf{a}^t)>0 ,\\
% %       -1 ; & \textrm{otherwise}.\\
% %     \end{array}
% % \right.
% % \end{equation}

% % \subsection{Generalization to Poisoning Attack}
% % Poisoning attack aims to perturb the data during training to lower the performance of model when testing. Its objective function is as follows:
% % \begin{equation}
% % \begin{split}
% %     &\max\mathcal{O}_a(\tilde{G}) = \mathcal{L}(f_{\theta^{*}_{\tilde{G}}}(\tilde{G}),\mathbf{z})\\
% %     &s.t.\ \mathcal{D}(G,\tilde{G})\leq\Delta_a,\ \theta^{*}_{\tilde{G}}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(\tilde{G}),\mathbf{z})
% % \end{split}
% % \end{equation}

% % As a defender, the objective function turns into following:
% % \begin{equation}
% % \begin{split}
% %     \min& \mathcal{O}_d(G_d) = \mathcal{D}(f_{\theta^{*}_{G}}(G),f_{\theta^{*}_{\tilde{G_d}}}(\tilde{G_d}))\\
% %     s.t.&\ \mathcal{D}(G,G_{d})\leq\Delta_d,\\
% %     & \mathcal{D}(G_d,\tilde{G_{d}})\leq\Delta_a,\\
% %     &\theta^{*}_{G}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(G),\mathbf{z})\\
% %     &\theta^{*}_{\tilde{G_d}}=\arg\min_{\theta}\mathcal{L}(f_{\theta}(\tilde{G_d}),\mathbf{z})\\
% %     &\tilde{G}_{d} = \arg\max\mathcal{O}_a(\tilde{G_d})
% %     % &G_{d} = \arg\max\mathcal{O}_a(G_d)
% % \end{split}
% % \end{equation}

% \subsection{Training Procedure and Implementation}
% The basic training strategy of our framework is to estimate the action-value function $Q(\mathbf{s}^t,\mathbf{a}^t)$ by gradient descent as many deep Q networks did~\cite{mnih2015human}. We also import commonly-used techniques to boost the training such as replay memory~\cite{mnih2015human} and probability $\epsilon$ which decays with training to balance the exploitation-exploration trade-off. In order to improve training efficiency, we use the trick mentioned at the end of Sec.~\ref{sec:problemDefinition} and relax $\theta^*_{G_d}$ as $\theta^*_{G}$. The loss function we selection is mean square error (MSE). As we mentioned before, from the perspective of a defender, we aim to select the most vulnerable unlabelled nodes as target nodes $\mathcal{V}_t$, and without adding computational complexity, the confidence of node classifier is a decent guide. Hence, for sampling target nodes $\mathcal{V}_t$, we adopt the weighted random sample whose weight is the entropy of the output of node classifier. The key idea of this entropy-weighted random sample strategy is that for a unlabelled node sample $v\in \mathcal{V}_u$, the less confident the node classifier towards it, the closer this node sample is embedded with decision boundary, the more fragile it is, and more likely to be protected by our framework. We summarize the whole training procedure of our proposed framework in Algorithm~\ref{alg:training procedure}.
% % In experiment section we illustrate that this strategy can greatly improve the robustness of the whole unlabelled node set. use the confidence of target classifier on test data $\mathcal{V}_u$ to evaluate the fragility of the unlabeled nodes and select the top-$k$ ambiguous nodes as the target nodes $\mathcal{V}_t$.

% \begin{algorithm}
% \caption{Training Procedure}
% \label{alg:training procedure}
% \SetAlgoLined
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \SetKwFunction{KwSimulation}{Simulation}
% \SetKwFunction{KwAttacker}{FGSM}
% \SetKwFunction{KwMSE}{MSE}
% \SetKwFunction{KwSample}{RandomSample}
% \SetKwFunction{KwWeightedSample}{Entropy-WeightedRandomSample}
% \SetKwFunction{KwRandomAction}{RandomAction}
% \SetKwFunction{KwRandomNumber}{RandomNumber}
% \SetKwFunction{KwPush}{Push}
% \SetKwProg{Fn}{Function}{}{}
% \Input{Benign graph $G$, simulated attacker \KwAttacker, label set $\mathcal{Y}$, discount factor $\gamma$, defense budget $\Delta_d$, exploitation-exploration trade-off probability $\epsilon$;}
% \Output{defense action-value function $Q$.}
%  initialization: obtain $\theta^*$ of GCN $f$ with $G$ and $\mathcal{Y}_l$; empty $memory$; random initialize parameters of $Q$ and node embedding model\;
%  \While{not converge}{
%   \KwSimulation\;
%   $\mathcal{V}_t,\mathbf{s}^t,\mathbf{s}^{t+1},\mathbf{a}^t,r\leftarrow$ \KwSample{$memory$}\;
%   $output\leftarrow\mathbf{W}^{(1)}\ \textrm{ReLU}(\mathbf{W}^{(0)}(\mathbf{s}^t||\mathbf{a}^t))$\;
%   $target\leftarrow r+\gamma\max_{\mathbf{a}^{t+1}}Q(\mathbf{s}^{t+1},\mathbf{a}^{t+1})$\;
%   $loss\leftarrow$  \KwMSE{$output,target$}\;
%   update parameters in $Q$ and node embedding model\;
%  }
 
% \BlankLine
% \Fn{\KwSimulation}{
%  $\mathcal{V}_t\leftarrow$\KwWeightedSample{$\mathcal{V}$}\;
%  $G^0_d\leftarrow G$\;
%  \For{$t\leftarrow 0$ \KwTo $\Delta_d-1$}{
%   compute $\mathbf{s}^t$ based on Eq.~\eqref{eq:state function} with $\mathcal{V}_t$ and $G^t_d$\;
%   \lIf{\KwRandomNumber $<\epsilon$}{$\mathbf{a}^t\leftarrow$\KwRandomAction}
%   \lElse{compute $\mathbf{a}^t$ based on Eq.~\eqref{eq:greedy selection} with $\mathbf{s}^t$}
%   generate actioned defended graph $G^{t+1}_d$\;
%   compute $\mathbf{s}^{t+1}$ based on Eq.~\eqref{eq:state function} with $\mathcal{V}_t$ and $G^{t+1}_d$\;
%   $\tilde{G^{t}_d}\leftarrow$\KwAttacker{$G^{t}_d$}\;
%   $\tilde{G^{t+1}_d}\leftarrow$\KwAttacker{$G^{t+1}_d$}\;
%   Obtain reward $r$ with Eq.~\eqref{eq:reward function} with $\tilde{G^{t}_d}, \tilde{G^{t+1}_d}, G$\;
%   $memory$.\KwPush{$\mathcal{V}_t,\mathbf{s}^t,\mathbf{s}^{t+1},\mathbf{a}^t,r$}\;
%  }
% }
 
% \end{algorithm}

==> Files/08Timeline.tex <==
\section{Timeline}
\begin{itemize}
    \item 9.13 - 9.19: Present all the updated experiments (e.g., added baselines) on overleaf.
    \item 9.13 - 9.26: Keep trying to verify the effectiveness of low-rank version. If work well, updated all the low-rank version-related methods and effectiveness/efficiency results on overleaf.
    \item 9.20 - 10.3: The first revised draft should be ready.
    \item 10.14 Abstract due.
    \item 10.21 Full paper due.
\end{itemize}

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX
